A Comprehensive Survey of Data Augmentation in Visual Reinforcement Learning

Visual reinforcement learning (RL), which makes decisions directly from high-dimensional visual inputs, has demonstrated significant potential in various domains. However, deploying visual RL techniques in the real world remains challenging due to their low sample efficiency and large generalization gaps. To tackle these obstacles, data augmentation (DA) has become a widely used technique in visual RL for acquiring sample-efficient and generalizable policies by diversifying the training data. This survey aims to provide a timely and essential review of DA techniques in visual RL in recognition of the thriving development in this field. In particular, we propose a unified framework for analyzing visual RL and understanding the role of DA in it. We then present a principled taxonomy of the existing augmentation techniques used in visual RL and conduct an in-depth discussion on how to better leverage augmented data in different scenarios. Moreover, we report a systematic empirical evaluation of DA-based techniques in visual RL and conclude by highlighting the directions for future research. As the first comprehensive survey of DA in visual RL, this work is expected to offer valuable guidance to this emerging field.

==> textfile/0ld_3.tex <==
\newpage
\section{How to Augment Data in Visual RL?} \label{How to augment the data in Visual RL?}
The aim of DA is to increase the amount and diversity of the original training data so that agents can learn more efficient and robust policies~\cite{svea}.
Thus, a primary focus of previous research was to design effective augmentation approaches~\cite{mixreg, playvirtual}.
In this section, we introduce the mainstream augmentation techniques and discuss the pros and cons of these methods.

\begin{figure}[ht] 
\centering
% \vspace{-0.2\baselineskip}
\includegraphics[width=\textwidth]{image/obs_tran_traj_augmentation.pdf}
% \vspace{-0.2\baselineskip}
\caption{
The comparison of different DA paradigms depending on the type of data augmented:
\textbf{observation augmentation} only generates synthetic observations $o_t^{aug}$;
\textbf{transition augmentation} augments observations together with supervision signals $(o_t^{a u g}, a_t^{a u g}, r_t^{a u g})$; and
\textbf{trajectory augmentation} generates virtual trajectories $(o_t^{a u g}, a_t^{{aug }}, o_{t+1}^{{aug }}, a_{t+1}^{a u g}, \ldots, o_{t+k}^{a u g})$.} 
\label{Overview of Section3} 
\end{figure}

\vspace{0.5\baselineskip}
In Figure~\ref{Overview of Section3}, we divide the DA approaches in visual RL into three main categories.
\textbf{Observation augmentation} only transforms the given observations and keeps the other transition factors (e.g., actions and rewards) unchanged, which is similar to the label-preserving perturbations in SL.
This kind of augmentation technique can be further categorized into two groups: classic image manipulations (Section~\ref{Classical Image Transformations for Observation Augmentation}) and deep neural network (DNN)-based transformations (Section~\ref{DNN-based Transformations for Observation Augmentation}).
The other two augmentation types, transition augmentation and trajectory augmentation, specifically consider the properties of RL to expand the scope of augmentation.
In Section~\ref{Transition Augmentation}, we introduce \textbf{transition augmentation}, which augments observations along with supervision signals such as rewards.
In Section~\ref{Trajectory Augmentation}, we discuss \textbf{trajectory augmentation} for generating synthesized sequential trajectories.
Furthermore, we present automatic augmentation (Section~\ref{Automatic Selection of Data Augmentation}) and task-aware augmentation (Section~\ref{Context-aware Data Augmentation}) as two extensions that are vital for achieving effective augmentation.

\subsection{Observation Augmentation via Classic Image Manipulations}
\label{Classical Image Transformations for Observation Augmentation}
A typical observation augmentation approach is to apply the classical image manipulations to the observed images; most such manipulations were originally proposed for computer vision applications.
Following the taxonomy of~\cite{image_aug_survey}, we identify five categories of image manipulations:
geometric transformations (Section~\ref{Geometric Transformation}),
photometric transformations (Section~\ref{Photometric Transformation}),
noise injections (Section~\ref{Noise Injection}),
random erasing (Section~\ref{Random Erasing})
and image mixing (Section~\ref{Mixing Images}).
Figure~\ref{aug} shows a list of the visualized examples.
\begin{figure}[ht]
\centering
% \vspace{-0.5\baselineskip}
\includegraphics[width=\textwidth]{image/AugTypes_long.pdf}
% \vspace{-0.5\baselineskip}
\caption{Visualized examples of observation augmentation via classical image manipulations.} 
\label{aug} 
\end{figure}

% \vspace{-0.5\baselineskip}
\subsubsection{Geometric Transformations}
\label{Geometric Transformation}
Geometric transformations are generally employed as optimality-invariant or label-preserving transformations~\cite{image_aug_survey} to overcome data shortages during the training process.
{\textbf{Random cropping}} is an effective preprocessing technique for improving data efficiency; it works on image data with mixed width and height dimensions by locating a random central patch in each frame with a specific dimensionality~\cite{drq, drq_v2}.
In many visual RL scenarios, such as robotic manipulation tasks, the vital regions are often positioned at the centers of the images, and cropping can remove irrelevant edge pixels to simplify the learning process~\cite{rad}.
Similar to cropping, the {\textbf{window}} transformation selects a random region and masks out the cropped part of the image, while {\textbf{translation}} renders the image with a larger frame and randomly moves the image within that frame.

\vspace{0.5\baselineskip}
Other forms of geometric transformation have also been introduced in visual RL scenarios.
For example, {\textbf{rotation}} involves rotating an image right or left by $r$ degrees, where $r$ is randomly selected from a range~\cite{rad};
{\textbf{flipping}} obtains additional data by flipping the observations horizontally or vertically.
Although these techniques have been proven effective in computer vision tasks such as ImageNet~\cite{image_aug_survey}, visual RL tasks are sensitive to angle information.
In such a scenario, transformations such as rotation and flipping may produce erroneous results without properly adjusting the corresponding actions.

\subsubsection{Photometric Transformations}
\label{Photometric Transformation}
In real-world applications, the colors of objects and backgrounds may vary due to conditions such as lighting and weather~\cite{AIReview_image_augmentation}.
The intuition behind photometric transformations is to simulate these color variations to prevent overfitting on the training data~\cite{overfitting_1, overfitting_2}.
Overfitting in visual RL is especially problematic due to the spurious correlations between task-irrelevant features and the agent’s policy, which can severely damage its test performance~\cite{observational_overfitting}.
Based on the prior knowledge concerning the variations between the training and test environments, photometric transformations aim to better generalize the agent’s policy to unseen visual environments.
For instance, {\textbf{grayscale}} simply converts images from RGB to grayscale~\cite{rad}, while {\textbf{color jitter}} varies the features of images that are commonly used in DA, including brightness, contrast, and saturation~\cite{autoaugment}.
A common way to perform jitter in the color space is to convert images from RGB to HSV and add noise to the HSV channels~\cite{rad}.
Furthermore, {\textbf{random convolution}} has been introduced to remove the visual bias that may damage the performance of convolutional neural networks (CNNs)~\cite{randfm}.
This approach augments the image color by passing the input observations through a random single-layer convolutional network, whose output layer has the same dimension as the input.

\subsubsection{Noise Injection}
\label{Noise Injection}
Adding noise to images can help CNNs learn robust features in computer vision tasks~\cite{noise},
and recent studies~\cite{svea, secant} also attempted to exploit this mechanism in visual RL to obtain robust state representations.
In practice, distortion can be introduced by adding {\textbf{Gaussian}} noise~\cite{rad} or {\textbf{impulse}} (salt-and-pepper) noise~\cite{secant}.

\subsubsection{Image Mixing}
\label{Mixing Images}
This type of methods is commonly used in computer vision tasks to improve a model’s robustness and generalization ability~\cite{why_mixup}.
Among the different versions of mixing, {\textbf{Overlay/Mixup}}~\cite{mixup} trains a neural network on the convex combinations of samples and their labels.
In visual RL, there are two ways to leverage the Mixup mechanism.
First, we can combine two observations and their supervision signals, which will be discussed in Section~\ref{Transition Augmentation}.
Alternatively, we can mix RL observations and other images randomly sampled from another dataset while the supervision signals of the observations remain fixed.
For example, SECANT~\cite{secant} linearly blends an observation with a distracting image $I$ as $f(o)=\alpha o + (1-\alpha) I$, where $I$ is randomly sampled from the COCO~\cite{coco} image set.

\subsubsection{Random Erasing}
\label{Random Erasing}
As an analog of the dropout regularization, erasing prevents the network from overfitting by working in the input data space instead of the network structure space~\cite{Random_Erasing}.
{\textbf{Cutout}}~\cite{cutout} partially erases an image by randomly masking an $m \times n$ patch of the image.
Furthermore, {\textbf{Cutout-Color}} masks the patch with a random color.
As a combination of Cutout and Mixup, {\textbf{CutMix}}~\cite{cutmix} replaces the removed region with a patch from another image and the supervision signals of the original observation are preserved (in visual RL scenarios)~\cite{secant}. 

\subsection{Observation Augmentation via DNN-based Transformations}
\label{DNN-based Transformations for Observation Augmentation}
In addition to classic image manipulation methods, a wide variety of augmentation techniques that leverage the properties of DNNs are available.
This subsection introduces the concepts of feature space augmentation, adversarial augmentation and generative adversarial network (GAN)-based augmentation in visual RL.

\subsubsection{Feature Space Augmentation}
\label{Feature space augmentation}
Instead of applying DA in the input space, another effective approach is to perform the transformation in the feature space~\cite{feature_space_augmentation}.
The feature space, also known as the latent or embedding space, refers to the abstract space that encodes meaningful internal representations from the original high-dimensional data.
The first solution is to use autoencoders to map input images to the latent feature space and then reconstruct the images based on the augmented features in the original space.
The augmentations performed in the latent space usually include Gaussian noise addition and linear interpolation~\cite{modals}, which can generate more diversified datasets than classic transformations in many supervised tasks~\cite{latent_space_interpolation, Auto-encoder-based_generative}.
Unfortunately, apart from a few studies that used autoencoders for designing reconstruction-based auxiliary tasks to facilitate representation learning~\cite{sac_ae, imagined_goals}, the use of autoencoders to obtain high-quality augmented data has yet to be explored in visual RL scenarios.

CLOP

\vspace{0.5\baselineskip}
Another solution is to extract representations from the bottom layers of a CNN and directly augment the latent data without reconstructing the high-dimensional images~\cite{image_aug_survey}.
For example, MixStyle~\cite{mixstyle} is an interesting technique that adopts style mixing in the bottom layers to simulate various visual styles~\cite{style_transfer} and has achieved proven cross-domain generalization performance on benchmarks such as CoinRun~\cite{CoinRun}.
Recently, CLOP~\cite{clop} was proposed as a novel augmentation technique that swaps the positions of pixels in the feature maps after the deepest convolutional layer while preserving the consistency across channels.
The experimental evaluation showed that CLOP achieves significant generalization performance improvement without requiring additional representation learning tasks due to the high-level abstract features contained in the deepest neural network layer.

\subsubsection{Feature Space AugmentationAdversarial Augmentation}
\label{Adversarial Augment}
Since DNNs are vulnerable to adversarial perturbations, training a model on adversarial samples can potentially enhance its generalization~\cite{adversarial_examples}.
Inspired by the success in SL~\cite{adversarial_da}, PADDA~\cite{padda} deploys an adversarial DA technique in RL by minimizing the expected reward that an RL agent intends to maximize.
Based on policy gradient algorithms, PADDA creates an adversarial sample $\left(\hat{s}_{t}, \hat{a}_{t}=a_{t}, \hat{r}_{t}=r_{t}\right)$ for each transition sample $(s_t, a_t, r_t)$:
\begin{equation}
    \hat{s}_{t}=\underset{s}{\operatorname{argmin}} \log \pi_{\theta}\left(a_{t} \mid s\right)\left(r_{t}-V(s)\right)+\gamma\left\|s-s_{t}\right\|^{2}
\end{equation}
where $\pi_{\theta}\left(a_{t} \mid s\right)$ is the policy function and $V\left(s_{t}\right)$ is the value function of state $s_{t}$~\cite{ppo}.
Furthermore, to stabilize the optimization process, PADDA constructs a new trajectory by randomly selecting appropriate transitions from the original and augmented trajectories.
In contrast to traditional augmentation techniques, adversarial augmentation specifically considers the features of RL.

\subsubsection{GAN-Based Augmentation}
\label{GAN-based Augmentation}
GAN-based augmentation is a popular augmentation methodology in supervised and unsupervised learning~\cite{gan-based_data_augmentation,AAAI22_GAN,GAN_based_data_augmentation2}.
However, it has yet to attract similar attention in visual RL; this is probably due to the difficulty of generating meaningful transitions.
A related study applied GAN-based image-to-image translation to map visual observations from the target domain to the source domain to address the challenge of transfer learning~\cite{image-to-image_translation}.
Instead of generating diverse training data, this approach applies an unaligned GAN to eliminate the distracting parts of the observations during the test process.
In general, how to leverage GANs to perform effective DA in visual RL remains an open question for future studies.

\subsection{Transition Augmentation}\label{Transition Augmentation}
As shown in Figure~\ref{mixreg}, augmenting $s_t$ with fixed supervision signals (e.g., the reward $r_t$ and action $a_t$) can be viewed as a kind of local perturbation of the corresponding transition.
To ensure the the validity of the augmented transition $<s_t^{aug}, a_t, r_t, s_{t+1}^{aug}>$, the augmented observation $s_t^{aug}$ is only allowed to be in the vicinity of $s_t$.
Hence, local perturbation is inherently limited in terms of increasing data diversity, which is a common issue faced by all observation augmentations.

\begin{figure}[ht] 
\centering 
\includegraphics[width=\textwidth]{image/Mixreg.pdf} 
\caption{Contrast between augmenting observations via local perturbations (left, Cutout-Color~\cite{cutout}) and augmenting observations along with the supervision signals through linear interpolation (right, MixReg~\cite{mixreg}).} 
\label{mixreg}
\end{figure}

An intuitive solution is to apply interpolation across different data points instead of performing a local perturbation on each individual data point.
Inspired by Mixup~\cite{mixup} and CutMix~\cite{cutmix}, MixReg~\cite{mixreg} convexly combines two observations and their supervision signals to generate augmented data.
For example, let $y_i$ and $y_j$ denote the signals for states $s_i$ and $s_j$, respectively, which can be the reward or state values. 
After interpolating the observations by $\tilde{s}=\lambda s_{i}+(1-\lambda) s_{j}$, MixReg introduces mixture regularization in a similar manner via $\tilde{y}=\lambda y_{i}+(1-\lambda) y_{j}$, which helps learn more effective representations and smoother policies.

\subsection{Trajectory Augmentation}\label{Trajectory Augmentation}
Since observation or transition augmentation cannot directly enrich the trajectories encountered during training, to further improve the sample efficiency,
PlayVirtual~\cite{playvirtual} augments the actions to generate synthesized trajectories under a self-supervised cycle consistency constraint.

\begin{figure}[ht] 
\centering 
\includegraphics[width=\textwidth]{image/Playvirtual.pdf} 
\caption{Data flow and architecture of PlayVirtual~\cite{playvirtual} as an example of trajectory augmentation.} 
\label{PlayVirtual}
\end{figure}

\vspace{0.5\baselineskip}
In Figure~\ref{PlayVirtual}, PlayVirtual operates entirely in the latent space after encoding the input observation $s_t$ into a low-dimensional state representation $z_t$.
Following the dynamics model (DM) in SPR~\cite{spr}, PlayVirtual introduces a backward dynamics model (BDM) to predict the backward transition dynamics $(z_{t+1},a_t) \longrightarrow z_t$ to build a loop with the forward trajectory.
During the training process, the DM is supervised by the original trajectory information, whereas the BDM is constrained by the cycle consistency between $z_t$ and $z^{\prime}_t$.
Further discussion on how to train the dynamics models with the auxiliary loss will be provided in Section~\ref{Policy Regularization Explicitly with Auxiliary Loss}.
After obtaining the effective DM and BDM, PlayVirtual can generate diverse synthesized trajectories by randomly sampling/augmenting $M$ sets of actions in the action space $\mathcal{A}$ and then calculating the state information.
Experimental studies confirmed that regularizing feature representation learning with cycle-consistent synthesized trajectories is the key to PlayVirtual's success.

\subsection{Automatic Augmentation}\label{Automatic Selection of Data Augmentation}

Automatic augmentation is receiving increasing attention due to the demand for task-specific augmentations~\cite{auto1,auto2,autoaugment}.
For example, although random cropping is one of the most effective augmentation techniques for improving sample efficiency on many benchmarks, such as DMControl-500k~\cite{rad,drq} and Procgen~\cite{drac}, the induced generalization ability improvement heavily depends on the specific choice of augmentation strategy.
Generally, different tasks benefit from different augmentations, and selecting the most appropriate DA approach requires expert knowledge.
Therefore, it is imperative to design a method that can automatically identify the most effective augmentation method.
The related research in visual RL is still in its infancy~\cite{drac}, and we report some promising approaches below.

\paragraph{{Upper Confidence Bound (UCB):}}
The task of selecting an appropriate augmentation from a given set can be formulated as a multi-armed bandit problem where the action space is the set of available transformations $F=\{f_1,f_2,\dots,f_n\}$.
The UCB~\cite{ucb} is a popular solution for the multi-armed bandit problem that considers both exploration and exploitation.
Recently, UCB-DrAC~\cite{drac} and UCB-RAD~\cite{UCB-RAD} were proposed to achieve automatic augmentation in visual RL.
The experiment results suggest that UCB-based automatic augmentations can significantly improve an agent's generalization capabilities.

\paragraph{{Meta Learning:}}
Meta learning is an alternative solution to automatic augmentation.
It can be implemented in two ways~\cite{drac}:
$(1)$ training a meta learner such as RL$^2$~\cite{rl2} to automatically select an augmentation type before every update in a DA-based algorithm;
$(2)$ meta learning the weights of a CNN to perturb the observed images, which is similar to model-agnostic meta learning (MAML)~\cite{maml,meta}.
In practice, both approaches have not yet produced sufficiently promising results, and it remains challenging to design expressive functions for automatic augmentation based on meta learning.

\subsection{Context-Aware Augmentation}
\label{Context-aware Data Augmentation}

\begin{wrapfigure}{l}{0.47\textwidth}
\centering
% \vspace{-\baselineskip}
\includegraphics[width=0.468\textwidth]{image/Context-agnostic_Transformation.pdf}
\caption{Context-agnostic augmentation.}
\label{Context-agnostic Augmentation}
\end{wrapfigure}
Another deficiency of current DA methods is that they rely on pixel-level image transformations, where each pixel is treated in a context-agnostic manner~\cite{tlda}.
However, in visual RL, the pixels in an observation are likely to have different levels of relevance to the decision making process~\cite{Visualizing_and_understanding, attention_augmented_agents}.
Figure~\ref{Context-agnostic Augmentation} shows that the context-agnostic augmentation may mask or destroy regions in the original observation that are vital for decision making.
This context-agnostic property explains why the naive application of prior-based strong augmentation may severely damage both the sample efficiency and the training stability of visual RL, regardless of its potential to enhance generalization~\cite{svea,tlda}.
Therefore, it is necessary to incorporate context awareness into augmentation, and two viable solutions are available for doing so.
\begin{enumerate}
\item \textbf{Introducing human guidance.}
Human-in-the-loop RL (HIRL)~\cite{HIRL} is a general paradigm that leverages human guidance to assist the RL process.
EXPAND~\cite{expand} introduces a human saliency map to mark the importance levels of different regions, and it only perturbs the irrelevant regions.
Saliency maps contain human domain knowledge, allowing context information to be embedded into the augmentation.
\item \textbf{Excavating task relevance.}
In visual RL, the contextual information can be extracted from the task relevance of each pixel, making it possible to directly determine its task relevance to achieve context-aware augmentation.
Task-aware Lipschitz DA (TLDA)~\cite{tlda} explicitly defines the task relevance by computing the Lipschitz constants produced when perturbing corresponding pixels.
Regions with large Lipschitz constants are crucial for the current task decision, and these regions will subsequently be protected from augmentation.
\end{enumerate}

Context-aware augmentation is the foundation for semantic-level DA, which is challenging and pivotal~\cite{keepaugment, tlda}.
In Section~\ref{Semantic-level Data Augmentation}, we will further discuss semantic-level DA as an important direction for future studies.
